DiaBLa: A Corpus of Bilingual Spontaneous Written Dialogues for Machine Translation

We present a new English-French test set for the evaluation of Machine Translation (MT) for informal, written bilingual dialogue. The test set contains 144 spontaneous dialogues (5,700+ sentences) between native English and French speakers, mediated by one of two neural MT systems in a range of role-play settings. The dialogues are accompanied by fine-grained sentence-level judgments of MT quality, produced by the dialogue participants themselves, as well as by manually normalised versions and reference translations produced a posteriori. The motivation for the corpus is two-fold: to provide (i) a unique resource for evaluating MT models, and (ii) a corpus for the analysis of MT-mediated communication. We provide a preliminary analysis of the corpus to confirm that the participants' judgments reveal perceptible differences in MT quality between the two MT systems used.

==> dialogue.tex <==
        
    \begin{tabular}{lrrr}
    \toprule
    & EN & FR & All  \\
    \midrule         
    \multicolumn{4}{c}{\#Turns}  \\ 
\midrule 
Total & 1,067 & 1,089 & 2,156 \\ 
Mean /dialogue & 7.4 & 7.6 & 15.0 \\ 
\midrule 
\multicolumn{4}{c}{\#Sentences}  \\ 
\midrule 
Total & 2,865 & 2,883 & 5,748 \\ 
Mean /dialogue & 19.9 & 20.0 & 39.9 \\ 
Min. /dialogue & 5 & 5 & 10 \\ 
Max. /dialogue & 42 & 60 & 102 \\ 
Mean /turn & 2.7 & 2.6 & 2.7 \\ 
Min. /turn & 1 & 1 & 1 \\ 
Max. /turn & 9 & 10 & 10 \\ 
\midrule 
\multicolumn{4}{c}{\#Tokens (original messages)}  \\ 
\midrule 
Total & 28,137 & 29,275 & 57,412 \\ 
Total unique & 3,471 & 4,058 & - \\ 
Mean /dialogue & 195.4 & 203.3 & 398.7 \\ 
Min. /dialogue & 67 & 54 & 121 \\ 
Max. /dialogue & 612 & 664 & 1,276 \\ 
Mean /sentence & 9.8 & 10.2 & 10.0 \\ 
Mode /sentence & 8 & 5 & 8 \\ 
Median /sentence & 8.0 & 9.0 & 9.0 \\ 
Min. /sentence & 1 & 1 & 1 \\ 
Max. /sentence & 46 & 52 & 52 \\ 
\midrule 
\multicolumn{4}{c}{\#Tokens (translated messages)}  \\ 
\midrule 
Total & 27,729 & 28,896 & 56,625 \\ 
Total unique & 3,115 & 3,727 & - \\ 
Mean /dialogue & 192.6 & 200.7 & 393.2 \\ 
Min. /dialogue & 54 & 69 & 123 \\ 
Max. /dialogue & 634 & 633 & 1,267 \\ 
Mean /sentence & 9.6 & 10.1 & 9.9 \\ 
Mode /sentence & 6 & 7 & 7 \\ 
Median /sentence & 9.0 & 9.0 & 9.0 \\ 
Min. /sentence & 1 & 1 & 1 \\ 
Max. /sentence & 47 & 74 & 74 \\ 
      
    \bottomrule      
    \end{tabular}
